HybridCite: A Hybrid Model for Context-Aware Citation Recommendation

Citation recommendation systems aim to recommend citations for either a complete paper or a small portion of text called a citation context. The process of recommending citations for citation contexts is called local citation recommendation and is the focus of this paper. Firstly, we develop citation recommendation approaches based on embeddings, topic modeling, and information retrieval techniques. We combine, for the first time to the best of our knowledge, the best-performing algorithms into a semi-genetic hybrid recommender system for citation recommendation. We evaluate the single approaches and the hybrid approach offline based on several data sets, such as the Microsoft Academic Graph (MAG) and the MAG in combination with arXiv and ACL. We further conduct a user study for evaluating our approaches online. Our evaluation results show that a hybrid model containing embedding and information retrieval-based components outperforms its individual components and further algorithms by a large margin.

==> 6_graphs.tex <==
\begin{figure}[tb]
\centering
 \includegraphics[keepaspectratio,width=0.8\linewidth]{figures/Approach/hd2vtrainflowchart2.pdf}
  \caption{Flowchart of the Hyperdoc2vec~\cite{ShiSZZH18} training process.}
  \label{fig:hd2vtraining}
\end{figure}

\begin{figure}[tb]
\centering
 \includegraphics[keepaspectratio, width=\linewidth]{figures/Approach/hd2v.pdf}
  \caption{Framework for the Hyperdoc2Vec~\cite{ShiSZZH18} model.}
  \label{fig:hd2v}
\end{figure}

\begin{table}[tb]
\centering
    \caption{Evaluation scores at k=10 for all models using the MAG50 data.}
    \label{tab:mag50evalk10}
\centering
\begin{small}
    \begin{tabular}{lllll}
    \toprule
    Model & MRR@10 & Recall@10 & MAP@10 & NDCG@10 \\
    \midrule
    hd2vOUT  & 0.1233 & 0.2200 & 0.1233 & 0.1660 \\
    BM25       & 0.1528 & 0.2836 & 0.1528 & 0.2082 \\
    hd2vINOUT & 0.0595 & 0.1353 & 0.1873 & 0.0898 \\
    Hybrid  & \textbf{0.1873} & \textbf{0.3760} & \textbf{0.1873} & \textbf{0.2711} \\
    LDA     & 0.0369 & 0.0892 & 0.0369 & 0.0567 \\
    Paper2Vec        & 0.0025 & 0.0113 & 0.0026 & 0.0055 \\
    \bottomrule
    \end{tabular}
    \end{small}
\end{table}

\begin{table}[tb]
    \centering
        \caption{Comparison of percentage of papers in ground truth (abbreviated as \textit{g.t.}) between Arxiv-MAG and MAG (number of cases in parentheses). ACL-MAG has only one ground truth in its contexts.}
    \label{tab:groundtruthscomparison}
    \begin{tabular}{lcccc}
    \toprule
    Data set & 1 g.t. paper \% & 2 g.t. papers \% & >2 g.t. papers \% \\
    \midrule
        MAG & 91.26\% (153953) & 6.04\% (10183) & 2.70\% (4564) \\
        Arxiv-MAG & 67.57\% (256037) & 16.96\% (64281) & 15.46\% (58599)\\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[keepaspectratio, width=\linewidth]{figures/Evaluation/MAG50MetricsGraphs2.pdf}
    \caption{Evaluation using MAG50: only papers with >= 50 citations in training set}
    \label{fig:mag50evaluation}
\end{figure}

\begin{figure}[tb]
    \centering
    \includegraphics[keepaspectratio, width=\linewidth]{figures/Evaluation/MAGCitedMetricGraphs2.pdf}
    \caption{Comparison of BM25 Evaluation for 2 MAG data sets: MAG and MAG-Cited.}
    \label{fig:magcitedevaluation}
\end{figure}

\begin{figure}[tb]
    \centering
    \includegraphics[keepaspectratio, width=\linewidth]{figures/Evaluation/MAGHybridv2metrics2.pdf}
    \caption{Comparing Hybrid23 with BM25 (MAG-Cited) and the original Hybrid algorithm.}
    \label{fig:maghybridevaluation}
\end{figure}


\begin{table}[tb]
\centering
    \caption{Comparing evaluation scores at k=10 for BM25 (MAG-Cited), Hybrid and Hybrid23}
    \label{tab:maghybridcited}
\centering
\begin{small}
    \begin{tabular}{lllll}
    \toprule
    Model & MRR@10 & Recall@10 & MAP@10 & NDCG@10 \\
    \midrule
    Hybrid  & 0.1422 & 0.3087 & 0.1414 & 0.2051 \\
    BM25 (MAG-Cited) & 0.2970 & 0.4769 & 0.2952 & 0.3777 \\
    Hybrid23  & \textbf{0.3056} & \textbf{0.5044} & \textbf{0.3035} & \textbf{0.3940} \\
    \bottomrule
    \end{tabular}
\end{small}
\end{table}


==> dataset.tex <==
\subsection{Evaluation Data Sets}
\label{sec:dataset}

The amount and quality of data used for training a machine learning model on real-world data is arguably more important than the quality of the actual algorithms used. Thus, the preparation of the input data is a critical step in the whole process. 
In the following sections, we will discuss our 4 'base' data sets, as well as the data preparation phase.

\subsubsection{Description of base data sets}
%Three data sources are used in this paper: MAG, Arxiv and ACL-ARC. 
The following three data sources are used in this paper. 
%% Details about the specific versions of the data sets that we use are given in Appendix~\ref{chap:offlineevalfilter}. These three 'base data sets' are described below.

\textbf{The MAG Data Set.}
The Microsoft Academic Graph (MAG) data set, a relatively new data set, has close to 220 million papers by 240 million authors (as of 22 May 2019). Papers in the data set range all the way from 1800 to 2019.\footnote{Latest statistics for Microsoft Academic can be found at https://academic.microsoft.com/home}

\textbf{ArXiv.}
arXiv\footnote{https://arxiv.org/} provides open access to the full text of papers from  mainly five disciplines -- mathematics, computer science, physics, biology, and economics. While citation contexts are not directly available, the full text in PDF as well as \LaTeX  files can be obtained from Arxiv. 

Although arViv does not quite match the breadth of coverage in MAG, it still contains a substantial number of papers. 
The total number of submissions, as of 22 May 2019, is over 1.5 million.\footnote{Current statistics are online available at \url{https://arxiv.org/stats/monthly\_submissions} and \url{https://arxiv.org/help/stats}.}

This paper uses the plain texts extracted from \TeX{} source files as provided by Saier and Färber~\cite{SaierF19}. 
In this way, in contrast to the MAG, we obtain full and clean text data. %%  from the arXiv data set. 

\textbf{ACL Anthology.}
The ACL Anthology Reference corpus (ACL-ARC) is a comparatively tiny dataset which covers only computational linguistics and natural language processing. It contains close to 11,000 papers and stretches from 1965 to 2006. The ACL data we use for this paper has been provided in a preprocessed format by \cite{Faerber2018}, containing sentences, reference information, and publications' metadata.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Data Set Preparation}
\label{sec:data-set-creation}

%%% We now discuss the data preparation step. 
The first step was to restrict the data sets to only computer science papers. Advantages to using only one discipline include likely better recommendations and reduced training time for embedding-based algorithms whilst missing out on cross-domain recommendations. 

The full-text base data sets (Arxiv and ACL-ARC) are supplemented with additional content from MAG. This content is made up of what is referred to in this paper as \textit{'pseudo full-text'}. The pseudo full-text for a paper consists of its title, abstract and all its citation contexts (i.e., citation contexts where it acts as a citing paper) from MAG.
Two additional data sets based on the MAG are created for evaluation: MAG50 and MAG-Cited. MAG50 is prepared the same way as the MAG data set, but with the added restriction that each of the papers must have been cited 50 times. MAG-Cited is a special data derived from MAG in which the title and abstract of each paper are combined with the citation contexts of papers which cite it to form alternative pseudo full-text. 

%% Assumming: not needed:
%% The end result is a single training file for each of the data sets. All the training files have citation markers of the form $=-=$MAG ID$-=-$, as all the papers in even the non-MAG data sets are mapped to MAG IDs.

%% NOW THE FOLLOWING TABLE IS COVERED BY THE TABLE "DETAILS ABOUT TRIANING AND TEST SETS"??!?
%%% Table~\ref{tab:MAGdatasets} contains some details about the training sets created for the MAG data sets (the main MAG data set, MAG50 and MAG-Cited). 

%Table~\ref{tab:nonmagdatasets} gives an overview of the training %sets created from the full-text data sets in conjunction with MAG %(pseudo full-text extracted from MAG).


% \todo{These details about the engineering are not necessary for the paper, so removed. Todo: Write short description (enumerate) of all used data sets, e.g., what MAG50 is. DONE}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if0
\textbf{Note about test set preparation}:
A test set containing citation contexts is also created for each of the data sets. All the test set citation contexts are extracted from the respective data source (Arxiv/ACL AAN/MAG), each of these test contexts must have at least 9 words after removing stop words. We remove stop words quite aggressively, based on \cite{StoneDK11}. All the stop words removed are given in \ref{chap:preprocessing}.



\subsubsection{MAG \textit{Pseudo full-text} preparation}
Since the MAG data set does not contain full text but contains citation contexts and plenty of metadata, a mechanism is needed to combine the contexts and metadata into a form usable by our algorithms. So, the title, abstract and citation contexts are retrieved for each paper and concatenated to form text which acts as a substitute, hence the name, \textit{pseudo full-text}. 

For each citation context, the MAG ID of its cited paper is inserted at its mid-point. The reason for this is that MAG citation data only contains one reference ID (cited paper ID) per citation context. If a citation context cites 2 papers, duplicate rows are present in the MAG citation data, each with one cited paper's reference ID associated with it.

In case of the non-MAG data sets, the papers are mapped to MAG, thereby enriching it with additional cited paper data where it was previously missing. Title, abstract and the citation contexts are retrieved and concatenated to form pseudo full-text. The reason we go through this process is that one of the embedding algorithms used (Hyperdoc2vec) requires representations for every citing and cited paper.

Pseudo full-text plays an important role in training all our algorithms. Table~\ref{tab:nonmagdatasets} shows that two of the prepared non-MAG data sets ultimately contain more pseudo full-text papers than full-text papers.

\subsubsection{MAG}
To prepare the MAG \textbf{training set}, the dump files are loaded into several PostgreSQL tables. From there, the pseudo full-text is prepared for each paper. A few other filter criteria are applied while preparing the training set. These filter criteria are explained in Appendix~\ref{chap:offlineevalfilter}.

The \textbf{test set} uses citation contexts from computer science papers in English which were published in 2018 and 2019.

The MAG citation data has a citing and cited MAG ID associated with each citation context. The cited MAG ID acts as the ground truth, duplicate data are grouped (by the paper id and the context) resulting in a single record with multiple cited papers in the ground truth. 

\subsubsection{Arxiv-MAG}
Saier et al. \cite{SaierF19} present an approach to convert \LaTeX source files provided by Arxiv into text files and create a database in which they map the papers in the reference section of each paper to MAG. They also obtain the precise positions of the citation markers corresponding to each of the references in the paper text, and insert placeholders with unique IDs at these locations.

These text files and the aforementioned mapping database act as the starting point for the preparation of the Arxiv-MAG \textbf{training file} in this paper. The MAG IDs from the references database are inserted at the positions in the Arxiv text files with unique IDs, replacing the citation placeholders. Arxiv provides a metadata file \footnote{https://arxiv.org/help/bulk\_data}, which is indexed in Apache Solr \footnote{https://lucene.apache.org/solr/} at this stage.

A couple of filter conditions are applied on the data set of Arxiv papers -- only computer science papers from 1991-2016 are considered and papers which have been cited less than five times are discarded. Appendix~\ref{chap:offlineevalfilter} shows all the filter criteria.

As our final data set will contain additional data from MAG (pseudo full-text), it is necessary to map all the Arxiv IDs to MAG IDs. All the Arxiv papers which cannot be mapped to MAG are therefore discarded in the training set. 

Pseudo full-text is fetched from the MAG tables for the cited papers which are not within the reduced Arxiv data set. This pseudo full-text includes only those citation contexts which cite papers within either the reduced Arxiv data set or the set of papers which the original Arxiv papers cite.

To prepare the \textbf{test set}, citation contexts of computer science papers from 2017 are extracted from Arxiv. Like in the training set, the Arxiv IDs of the cited papers are mapped to MAG IDs, and act as the ground truth. Again, references which are not in the training set are discarded from the ground truth.

\subsubsection{ACL-MAG}
In \cite{Faerber2018b} and \cite{Faerber2018}, the authors describe a method to detect citation contexts from ACL Anthology (and Arxiv) papers. They also provide the data for \cite{Faerber2018b} online \footnote{\url{http://citation-recommendation.org/publications/}}. They have obtained the references of each paper and mapped them to GC/DBLP. The data has been divided into 3 files for each paper: a text file containing text and annotations for citation markers, a references file, and a metadata file. 

To create the \textbf{training set}, we make use of just the text files and consider only the annotations which have been mapped to DBLP. The DBLP URL is obtained from the DBLP annotations and scraped to obtain the paper's title. This title is used to map to MAG in the same way as for Arxiv. The annotations are replaced by the MAG IDs to obtain the full text. The training data contains all papers from 1965 to 2005.
Again, additional MAG pseudo-text is added for these papers' reference papers.

The \textbf{test set} contains contexts from ACL Anthology papers in 2006. The papers in the ground truth are fetched from the references and mapped to MAG in the same way as the training set. Any papers not in the training set are removed from the ground truth. Unlike Arxiv, all the test set contexts have only one paper in the ground truth. 

\subsubsection{MAG-50}
The data preparation is very similar to the normal MAG data set (see Appendix~\ref{chap:offlineevalfilter}), but only papers with at least 50 citations are included in the training set. This means that papers with few citations, e.g. newly published papers, will never get recommended. This data set is used for comparison and analysis purposes. It is also used in the final recommender system.

\subsubsection{MAG with cited contexts (MAG-Cited)}
\cite{HuangKCMGR12} and \cite{Huang2015} claim that "a citation’s context contains explicit words explaining the citation". Meaning the words in the context explain the cited paper rather than the citing paper. This paper tries to verify this claim by creating an alternative data set where MAG file use citation contexts from papers which cite the paper instead of each paper's own citation contexts in its pseudo full-text.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
